Spider 2.0: Evaluating Language Models on Real-World Enterprise Text-to-SQL Workflows

Real-world enterprise text-to-SQL workflows often involve complex cloud or local data across various database systems, multiple SQL queries in various dialects, and diverse operations from data transformation to analytics. We introduce Spider 2.0, an evaluation framework comprising 632 real-world text-to-SQL workflow problems derived from enterprise-level database use cases. The databases in Spider 2.0 are sourced from real data applications, often containing over 1,000 columns and stored in local or cloud database systems such as BigQuery and Snowflake. We show that solving problems in Spider 2.0 frequently requires understanding and searching through database metadata, dialect documentation, and even project-level codebases. This challenge calls for models to interact with complex SQL workflow environments, process extremely long contexts, perform intricate reasoning, and generate multiple SQL queries with diverse operations, often exceeding 100 lines, which goes far beyond traditional text-to-SQL challenges. Our evaluations indicate that based on o1-preview, our code agent framework successfully solves only 21.3% of the tasks, compared with 91.2% on Spider 1.0 and 73.0% on BIRD. Our results on Spider 2.0 show that while language models have demonstrated remarkable performance in code generation -- especially in prior text-to-SQL benchmarks -- they require significant improvement in order to achieve adequate performance for real-world enterprise usage. Progress on Spider 2.0 represents crucial steps towards developing intelligent, autonomous, code agents for real-world enterprise settings. Our code, baseline models, and data are available at https://spider2-sql.github.io

==> colorboxdefs.tex <==
\newtcolorbox{observationbox}[1][]{
        colback=envfill,
        colbacktitle=envfill,
        colframe=envborder,
        arc=5pt,
        fontupper=\small,
        fonttitle=\bfseries\color{black},
        boxrule=0.5mm,
        boxsep=1mm,
        width=\linewidth,
        breakable,
        title={Observation \hfill #1},
        rounded corners,
        toptitle=0.7mm,
        bottomtitle=0.7mm
}
\newtcolorbox{goldpatchbox}[1][]{
        colback=goldpatchfill,
        colbacktitle=goldpatchfill,
        colframe=goldpatchborder,
        arc=5pt,
        fontupper=\small,
        fonttitle=\bfseries\color{black},
        boxrule=0.5mm,
        boxsep=1mm,
        width=\linewidth,
        breakable,
        title={Gold Patch \hfill #1},
        rounded corners,
        toptitle=0.7mm,
        bottomtitle=0.7mm
}
\newtcolorbox{issuebox}[1][]{
        colback=issuefill,
        colbacktitle=issuefill,
        colframe=issueborder,
        arc=5pt,
        fontupper=\small,
        fonttitle=\bfseries\color{black},
        boxrule=0.5mm,
        boxsep=1mm,
        width=\linewidth,
        breakable,
        title={Issue \hfill #1},
        rounded corners,
        toptitle=1mm
}
\newtcolorbox{agentbox}[1][]{
        colback=agentfill,
        colbacktitle=agentfill,
        colframe=agentborder,
        arc=5pt,
        fontupper=\small,
        fonttitle=\bfseries\color{black},
        boxrule=0.5mm,
        boxsep=1mm,
        width=\linewidth,
        breakable,
        title={SWE-agent \hfill #1},
        rounded corners,
        toptitle=1mm,
        lower separated=false
}
\newtcolorbox{fileviewerbox}[1]{
        enhanced,
        breakable,
        boxrule = 1.5pt,
        fontupper = \small,
        fonttitle = \bf\color{black},
        arc = 5pt,
        rounded corners,
        colframe = black,
        colbacktitle = swecream,
        colback = swecream,
        title = #1,
        left=4pt % moves left over a bit to make text never overlaps with border
}
\newtcolorbox{promptbox}[1]{
    enhanced,
    breakable,
    boxrule=1pt,  % Reduced from 1.5pt for a slimmer border
    fontupper=\small,
    fonttitle=\bfseries\color{black},
    arc=3pt,  % Reduced curvature for sharper corners
    rounded corners,
    colframe=black,
    colbacktitle=swecream,
    colback=swecream,
    title=#1,
    left=2mm,  % Reduce inner left margin
    right=2mm,  % Reduce inner right margin
    top=1mm,  % Reduce inner top margin
    bottom=1mm  % Reduce inner bottom margin
}


==> tables/main_result.tex <==
\begin{table*}[ht]
% \vspace{-15pt}
\centering
\caption{
Success rate (SR) of different frameworks and models on \ours, grouped by difficulty level. The costs under different settings are shown in Tab.\ref{tab:api-cost}.
}
\label{tab:exp_baseline}
\small
\scalebox{1}{
\renewcommand{\arraystretch}{1.1} % Increase the row height
\begin{tabularx}{\linewidth}{>{\centering\arraybackslash}p{2.1cm}>{\centering\arraybackslash}p{2.7cm}>{\centering\arraybackslash}X}
\toprule
\multirow{2}{*}{\textbf{Framework}} & \multirow{2}{*}{\textbf{Model}} & \textbf{Overall SR ($\uparrow$)} \\ 
\midrule
AutoEval & GPT-4o & 5.70\%  \\ \midrule
Reflexion & GPT-4o & 7.28\%  \\ \midrule 
CodeR & GPT-4o & 7.91\%  \\ \midrule   
Spider-Agent & o1-Preview   & \textbf{17.01\%}  \\
& GPT-4o   & 10.13\%  \\
& Claude-3.5-Sonnet & 9.02\%  \\
& GPT-4 &  8.86\% \\
& Qwen2.5-72B    & 6.17\%  \\
& DeepSeek-V2.5  & 5.22\%  \\
& Gemini-Pro-1.5 & 2.53\%  \\
& Llama-3.1-405B & 2.21\%  \\
\bottomrule
\end{tabularx}
}
\vspace{-10pt}
\end{table*}


% 
% o1preview 28.12 15.41 10.36 17.01
% gpt4o 16.88 10.04 4.66 10.13
% gpt4 20.63  7.17  1.55  8.86  33,20,3
% qwen                     23  13  3
% deepseek 13.13 3.23 1.55  21 9 3
% coder   13.75  7.17  2.59  7.43         23 22 5
% autoeval                                18 14 4
% reflexion                               23 21 2
% claude。                                23 26 8
% 
%21+17+4
% 26 23 5
% 26 21 2
% 160,279,193

==> tables/main_result_lite.tex <==





% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[]
\centering
\caption{
EX of baseline methods on \ours-lite, grouped by task categories: Cloud query, Local query and Snowflake. See Appendix for more details.}
\label{tab:lite-result}
\begin{tabular}{@{}lllll@{}}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Method}}} & \multicolumn{4}{c}{\textbf{EX (↑)}}                          \\ \cmidrule(l){2-5} 
\multicolumn{1}{c}{}                                 & Cloud Query     & Local Query & Snowflake & \textbf{Overall} \\ \midrule
DIN-SQL + GPT-4o                                     & 3.36\%          & -\%         & -\%       & -\%              \\ \midrule
DAIL-SQL + GPT-4o                                    & \textbf{4.69\%} & -\%         & -\%       & -\%              \\ \midrule
CHESS                                                & 3.36\%          & -\%         & -\%       & -\%              \\ \midrule
% CodeS-7B                                             & -\%             & -\%         & -\%       & -\%              \\ \midrule
% CodeS-13B                                            & -\%             & -\%         & -\%       & -\%              \\ \midrule
SFT CodeS-7B                                         & 0.69\%          & -\%         & -\%       & -\%              \\ \bottomrule
\end{tabular}
\end{table}




==> tables/spider2_overall_stat.tex <==
\begin{table*}[t]
\centering
\setlength\tabcolsep{2pt}
\resizebox{\textwidth}{!}{
\begin{tabular}{llll}  
\toprule  
\textbf{Benchmark} & \textbf{Fields} & \textbf{Ent. Serv.?} & \textbf{\# Tasks} \\
\hline  
DS-1000 \citep{lai2023ds1000}            & Code Completion &  &  \\
Arcade \citep{yin2023arcade}            & Notebook Completion &  &  \\
MLAgentBench \citep{huang2023mlagentbench}       & ML Project &  &  \\
DA-Bench \citep{hu2024dabench}           & CSV Analysis &  &  \\
Spider 2.0             & Data Analysis Project &  &  \\
\bottomrule  
\end{tabular}
    }
\caption{Comparisons of Spider 2.0 with other code generation benchmarks.}
    \vspace{-15pt}
\label{tab:benchmark_comparisons}%
\end{table*}%
